Dynamics of Parallel Manipulators with Hybrid Complex Limbs -- Modular Modeling and Parallel Computing

Parallel manipulators, also called parallel kinematics machines (PKM), enable robotic solutions for highly dynamic handling and machining applications. The safe and accurate design and control necessitates high-fidelity dynamics models. Such modeling approaches have already been presented for PKM with simple limbs (i.e. each limb is a serial kinematic chain). A systematic modeling approach for PKM with complex limbs (i.e. limbs that possess kinematic loops) was not yet proposed despite the fact that many successful PKM comprise complex limbs. This paper presents a systematic modular approach to the kinematics and dynamics modeling of PKM with complex limbs that are built as serial arrangement of closed loops. The latter are referred to as hybrid limbs, and can be found in almost all PKM with complex limbs, such as the Delta robot. The proposed method generalizes the formulation for PKM with simple limbs by means of local resolution of loop constraints, which is known as constraint embedding in multibody dynamics. The constituent elements of the method are the kinematic and dynamic equations of motions (EOM), and the inverse kinematics solution of the limbs, i.e. the relation of platform motion and the motion of the limbs. While the approach is conceptually independent of the used kinematics and dynamics formulation, a Lie group formulation is employed for deriving the EOM. The frame invariance of the Lie group formulation is used for devising a modular modeling method where the EOM of a representative limb are used to derived the EOM of the limbs of a particular PKM. The PKM topology is exploited in a parallel computation scheme that shall allow for computationally efficient distributed evaluation of the overall EOM of the PKM. Finally, the method is applied to the IRSBot-2 and a 3\underline{R}R[2RR]R Delta robot, which is presented in detail.

==> abstract_final.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,PKMComplexLoops_Kinematics.tex}
                      

Parallel manipulators, also called parallel kinematics machines (PKM),
enable robotic solutions for highly dynamic handling and machining
applications. The safe and accurate design and control necessitates
high-fidelity dynamics models. Such modeling approaches have already been
presented for PKM with simple limbs (i.e. each limb is a serial kinematic
chain). A systematic modeling approach for PKM with complex limbs (i.e.
limbs that possess kinematic loops) was not yet proposed despite the fact
that many successful PKM comprise complex limbs.

This paper presents a systematic modular approach to the kinematics and
dynamics modeling of PKM with complex limbs that are built as serial
arrangement of closed loops. The latter are referred to as hybrid limbs, and
can be found in almost all PKM with complex limbs, such as the Delta robot.
The proposed method generalizes the formulation for PKM with simple limbs by
means of local resolution of loop constraints, which is known as constraint
embedding in multibody dynamics. The constituent elements of the method are
the kinematic and dynamic equations of motions (EOM), and the inverse
kinematics solution of the limbs, i.e. the relation of platform motion and
the motion of the limbs. While the approach is conceptually independent of
the used kinematics and dynamics formulation, a Lie group formulation is
employed for deriving the EOM. The frame invariance of the Lie group
formulation is used for devising a modular modeling method where the EOM of
a representative limb are used to derived the EOM of the limbs of a
particular PKM. The PKM topology is exploited in a parallel computation
scheme that shall allow for computationally efficient distributed evaluation
of the overall EOM of the PKM. Finally, the method is applied to the
IRSBot-2 and a 3\underline{R}R[2RR]R Delta robot, which is presented in
detail.

\textit{Keywords--Parallel kinematics machines, parallel robots, complex
limbs, hybrid robots, dynamics, kinematics, control, screws, Lie group }$%
SE\left( 3\right) $, \textit{\ parallel computing}

